Determination of the theory uncertainties from missing higher orders on NNLO parton distributions with percent accuracy

We include uncertainties due to missing higher order corrections to QCD computations (MHOU) used in the determination of parton distributions (PDFs) in the recent NNPDF4.0 set of PDFs. We use our previously published methodology, based on the treatment of MHOUs and their full correlations through a theory covariance matrix determined by scale variation, now fully incorporated in the new NNPDF theory pipeline. We assess the impact of the inclusion of MHOUs on the NNPDF4.0 central values and uncertainties, and specifically show that they lead to improved consistency of the PDF determination with an ensuing moderate reduction of PDF uncertainties at NNLO.

==> tables/Table_B1.tex <==
\begin{tabularx}{\textwidth}{Xrcrc}
  \toprule
  \multirow{2}{*}{Dataset}
  & \multicolumn{2}{c}{NNPDF4.0}
  & \multicolumn{2}{c}{NNPDF4.0\_CUTS}  \\
  & $N_{\rm dat}$ & $\chi^2/N_{\rm dat}$
  & $N_{\rm dat}$ & $\chi^2/N_{\rm dat}$ \\
  \midrule
  DIS NC
  & 2100 & 1.23
  & 1613 & 1.14 \\
  DIS CC
  &  989 & 0.90
  &  552 & 0.89 \\
  DY NC
  &  &
  &  584 & 1.52 \\
  DY CC
  & &
  &  158 & 1.49 \\
  Top-quark pair production
  &   64 & 1.21
  &   64 & 1.25 \\
  Single-inclusive jet production
  &  356 & 0.96
  &  356 & 0.96 \\
  Di-jet production
  &  144 & 2.03
  &  144 & 1.98 \\
  Prompt photon production
  &   53 & 0.74 
  &   53 & 0.74 \\
  Single top-quark production
  &   17 & 0.36
  &   17 & 0.37 \\
  \midrule
  Total
  & 4616 & 1.17
  & 3541 & 1.21 \\
\bottomrule
\end{tabularx}

